Enhanced Convolutional Neural Tangent Kernels

Recent research shows that for training with $\ell_2$ loss, convolutional neural networks (CNNs) whose width (number of channels in convolutional layers) goes to infinity correspond to regression with respect to the CNN Gaussian Process kernel (CNN-GP) if only the last layer is trained, and correspond to regression with respect to the Convolutional Neural Tangent Kernel (CNTK) if all layers are trained. An exact algorithm to compute CNTK (Arora et al., 2019) yielded the finding that classification accuracy of CNTK on CIFAR-10 is within 6-7% of that of that of the corresponding CNN architecture (best figure being around 78%) which is interesting performance for a fixed kernel. Here we show how to significantly enhance the performance of these kernels using two ideas. (1) Modifying the kernel using a new operation called Local Average Pooling (LAP) which preserves efficient computability of the kernel and inherits the spirit of standard data augmentation using pixel shifts. Earlier papers were unable to incorporate naive data augmentation because of the quadratic training cost of kernel regression. This idea is inspired by Global Average Pooling (GAP), which we show for CNN-GP and CNTK is equivalent to full translation data augmentation. (2) Representing the input image using a pre-processing technique proposed by Coates et al. (2011), which uses a single convolutional layer composed of random image patches. On CIFAR-10, the resulting kernel, CNN-GP with LAP and horizontal flip data augmentation, achieves 89% accuracy, matching the performance of AlexNet (Krizhevsky et al., 2012). Note that this is the best such result we know of for a classifier that is not a trained neural network. Similar improvements are obtained for Fashion-MNIST.

==> intro_old.tex <==
%Inductive bias: decrease the complexity via model: weight sharing, via changing neural network architectures
Modern deep learning methods impose inductive bias to  improve the performance, based on prior knowledge about data.
For neural network models, a common way to impose inductive bias is to manipulate the architectures.
For example, convolutional neural networks (CNNs) use the same filter acting all patches (spatial weight sharing) to utilize the similarity among closer patches and recurrent neural networks use hidden states to keep long term relation.
%\simon{Check what is the formal way of saying these.}

%Global average pooling: CNN, CNN-GP, CNTK
% quotes NIN paper, only intuition, no justification
In this paper we study a particular component in modern convolutional models, global average pooling (\gap), first proposed in \cite{lin2013network}.
This operation is simple.
Before executing the final fully-connected layer, \gap~averages of the outputs of all patches from the last convolutional layer.
Nowadays, \gap~ has become a must-have in state-of-the-art CNNs for various computer vision tasks.
Furthermore, the success of \gap~ is in some sense universal.
Recently, \citet{novak2018bayesian,arora2019exact} found \gap~ can improve the performance of convolutional Gaussian process kernel (\cnngp) and convolutinal neural tangent kernel (\cntk).
 \footnote{See Section~\ref{sec:rel} for background and Section~\ref{sec:pre} for definitions of \cnngp and \cntk.}


%Raising the question
What is the reason behind the success of \gap?
A common folklore is that using \gap followed a fully-connected layer has fewer parameters to train than direct using a fully-connected layer.
However, modern neural networks are highly over-parameterized, i.e., they have more parameters than the training data, even with \gap.
Therefore,  parameter counting cannot explain why certain architecture generalize better than others~\citep{zhang2016understanding}.
Another hypothesis is that \gap~sums out the spatial information, thus it is more robust to spatial translations of the input~\citep{lin2013network}.
While this hypothesis makes intuitive sense, to our knowledge, there is no formal justification that even the meaning of ``robust to spatial translations has not been clearly stated.
To study this problem, we connect \gap~to data augmentation which is another way of imposing inductive bias.


%induvtive bias via data augmentation: a direct approach
Data augmentation is a more direct way of enforcing prior knowledge about the data.
The most common data augmentation schemes in computer vision are through translation and flip.
For image classification task, translating some pixels or flipping the input image  should not change the label.
Therefore, one can create more data by adding translated and flipped images  to the training set with labels as the original ones, then train a classifier on the new augmented training set.
\footnote{Note the new data can be created in an online fashion during stochastic gradient training.}
This simple scheme is quite effective for image classification task that ,ost state-of-the-art methods use this scheme.
%History of data augmentation theory
Theoretically, the study of data augmentation dates back to \cite{chapelle2001vicinal}.
When the underlying data generating process does have certain invariance, then data augmentation can reduce the sample complexity.
See \cite{chen2019invariance,dao2018kernel} for recent advance.

%why we build this connection
The current paper formally establishes the connection between \gap~and the full translation data augmentation scheme.\footnote{Full translation data augmentation: performing all possible translations. See Section~\ref{sec:pre} for the formal definition}
This connection will help us understand better about the benefit of \gap~and more importantly, its problem.
We make the following contributions:\begin{itemize*}
\item We show for \cnngp and infinitely wide CNN trained by gradient flow, a.k.a \cntk, with fully-connected layer as the last layer and full translation data augmentation is \emph{equivalent} to those with \gap, modulo boundary effects.
Our proof technique can be viewed as a successful application of the kernel view of neural networks. 
%gap and data aug
\item We derive a new formula to efficiently implement flip data augmentation in both training and test time for kernel predictors.
%kernel formula for flip
\item We observe that full translation can create unrealistic images (see Figure~\ref{fig...}) and we conjecture this phenomenon degrades the performance of the classifier.
We thus propose a new operation before the last layer, local average pooling (\lap), which corresponds to partial translation data augmentation.
Through extensive experiments on CIFAR 10 and fashion MNIST, we found \lap~consistently improve the performance of \cnn, \cnngp, \cntk.
In particular, we find \cnngp~with \lap~achieves $81\%$ on CIFAR 10 dataset, outperforming the best previous kernel predictor by $4\%$.
When using the proprosessing technique proposed by~\citet{coates2011analysis}, \cnngp~with \lap achieves $89\%$ accuracy, matching the performance of AlexNet~\citep{krizhevsky2012imagenet} and is the strongest non deep neural network classifier.
\end{itemize*}



\paragraph{Organization}
In Section~\ref{sec:rel}, we review related work.
In Section~\ref{sec:pre}, we introduce necessary notations and review \cnngp and \cntk.
In Section~\ref{sec:gap}, we establish the connection between \gap and translation data augmentation and discuss how to implement flip data augmentation for kernel predictor efficiently.
In Section~\ref{sec:lap}, we introduce \lap for \cnngp, \cntk and CNNs.
In Section~\ref{sec:exp}, we conduct extensive experiments on CIFAR 10 and Fashion-MNIST datasets to illustrate the effectiveness of \lap.
We conclude in Section~\ref{sec:con} and defer proofs and additional experiments to appendix.
